Enhancing Quantum-ready QUBO-based Suppression for Object Detection with Appearance and Confidence Features

Quadratic Unconstrained Binary Optimization (QUBO)-based suppression in object detection is known to have superiority to conventional Non-Maximum Suppression (NMS), especially for crowded scenes where NMS possibly suppresses the (partially-) occluded true positives with low confidence scores. Whereas existing QUBO formulations are less likely to miss occluded objects than NMS, there is room for improvement because existing QUBO formulations naively consider confidence scores and pairwise scores based on spatial overlap between predictions. This study proposes new QUBO formulations that aim to distinguish whether the overlap between predictions is due to the occlusion of objects or due to redundancy in prediction, i.e., multiple predictions for a single object. The proposed QUBO formulation integrates two features into the pairwise score of the existing QUBO formulation: i) the appearance feature calculated by the image similarity metric and ii) the product of confidence scores. These features are derived from the hypothesis that redundant predictions share a similar appearance feature and (partially-) occluded objects have low confidence scores, respectively. The proposed methods demonstrate significant advancement over state-of-the-art QUBO-based suppression without a notable increase in runtime, achieving up to 4.54 points improvement in mAP and 9.89 points gain in mAR.

==> sec/tables.tex <==
\setlength\tabcolsep{0.75mm} 
\begin{table}
    \centering
    \caption{Faster R-CNN, COCO2017 (4980 images)}
    \begin{tabular}{l r ccccc}
    \toprule
    \multicolumn{2}{c}{Metric} & NMS & S-NMS & QSQS & QAQS & QAQS-2 \\
    \midrule 
    Runtime (s)&($\downarrow$)& \textbf{83.09} & 103.01 & 134.42 & 150.95 & 150.31 \\ 
    % Time/Image (s)&($\downarrow$)& 0.017 & 0.021 & 0.027 & 0.059 & 0.058 \\ 
    % Solver time (s)&($\downarrow$)& - & - & 73.35 & 90.10 & 91.37 \\ 
    \midrule        
    OC cost    &($\downarrow$)& 31.70 &  33.62 &  \textbf{30.99} &  32.96 &  35.33 \\
    \midrule        
    mAP        & ($\uparrow$) & 34.61 &  35.20 &  34.04 &  34.89 &  \textbf{35.24} \\
    mAP@50     & ($\uparrow$) & 54.08 &  55.27 &  52.94 &  54.60 &  \textbf{55.33} \\
    mAP@75     & ($\uparrow$) & 37.69 &  \textbf{38.14} &  37.19 &  37.88 & 38.13 \\
    mAP@small  & ($\uparrow$) & 14.70 &  \textbf{14.82} &  14.63 &  14.68 &  \textbf{14.82} \\
    mAP@medium & ($\uparrow$) & 33.22 &  33.78 &  32.91 &  33.54 &  \textbf{33.90} \\
    mAP@large  & ($\uparrow$) & 45.68 &  \textbf{46.61} &  44.43 &  46.07 &  46.60 \\
    \midrule 
    mAR@1      & ($\uparrow$) & \textbf{29.26} &  \textbf{29.26} &  28.92 &  29.20 &  29.24 \\
    mAR@10     & ($\uparrow$) & 42.73 &  43.92 &  42.13 &  43.46 &  \textbf{44.21} \\
    mAR@100    & ($\uparrow$) & 43.79 &  45.22 &  42.90 &  44.53 &  \textbf{45.63} \\
    mAR@small  & ($\uparrow$) & 22.37 &  22.91 &  22.10 &  22.47 &  \textbf{23.16} \\
    mAR@medium & ($\uparrow$) & 43.18 &  44.55 &  42.47 &  43.80 &  \textbf{44.91} \\
    mAR@large  & ($\uparrow$) & 53.85 &  55.70 &  52.14 &  54.89 &  \textbf{56.17} \\
    \bottomrule
    \end{tabular}
\end{table}

\setlength\tabcolsep{0.75mm} 
\begin{table}
    \centering
    \caption{Faster R-CNN, CrowdHuman (4370 images)}
    \begin{tabular}{l r ccccc}
    \toprule
    \multicolumn{2}{c}{Metric} & NMS & S-NMS & QSQS & QAQS & QAQS-2 \\
    \midrule 
    Runtime (s)&($\downarrow$)& \textbf{182.24} & 241.48 & 183.63 & 184.36 & 174.15 \\ 
    % Time/Image (s)&($\downarrow$)& 0.042 & 0.055 & 0.042 & 0.18 & 0.17 \\ 
    % Solver time (s)&($\downarrow$)& - & - & 87.51 & 83.67 & 81.82 \\ 
    \midrule        
    OC cost    &($\downarrow$)&  \textbf{22.72} &  24.89 &  22.82 &  23.40 &  27.23 \\
    \midrule        
    mAP        & ($\uparrow$) &  34.01 &  34.97 &  31.23 &  35.04 &  \textbf{35.72} \\
    mAP@50     & ($\uparrow$) &  58.47 &  61.23 &  53.28 &  60.72 &  \textbf{62.48} \\
    mAP@75     & ($\uparrow$) &  35.09 &  35.68 &  32.32 &  35.74 &  \textbf{36.15} \\
    mAP@small  & ($\uparrow$) &   9.72 &   9.94 &   9.42 &   9.88 &  \textbf{10.09} \\
    mAP@medium & ($\uparrow$) &  29.16 &  29.93 &  27.11 &  29.66 &  \textbf{30.39} \\
    mAP@large  & ($\uparrow$) &  48.50 &  50.62 &  43.79 &  50.66 &  \textbf{51.61} \\
    \midrule 
    mAR@1      & ($\uparrow$) &   \textbf{3.36} &   \textbf{3.36} &   3.34 &   \textbf{3.36} &  \textbf{ 3.36} \\
    mAR@10     & ($\uparrow$) &  24.01 &  24.09 &  23.38 &  24.38 &  \textbf{24.44} \\
    mAR@100    & ($\uparrow$) &  39.77 &  41.92 &  36.19 &  41.44 &  \textbf{42.78} \\
    mAR@small  & ($\uparrow$) &  16.41 &  17.10 &  15.55 &  16.83 &  \textbf{17.75} \\
    mAR@medium & ($\uparrow$) &  37.00 &  38.61 &  33.86 &  38.07 &  \textbf{39.52} \\
    mAR@large  & ($\uparrow$) &  54.03 &  57.42 &  48.66 &  56.90 &  \textbf{58.33} \\
    \bottomrule
    \end{tabular}
\end{table}


























